Speaker-Independent Acoustic-to-Articulatory Inversion through Multi-Channel Attention Discriminator

We present a novel speaker-independent acoustic-to-articulatory inversion (AAI) model, overcoming the limitations observed in conventional AAI models that rely on acoustic features derived from restricted datasets. To address these challenges, we leverage representations from a pre-trained self-supervised learning (SSL) model to more effectively estimate the global, local, and kinematic pattern information in Electromagnetic Articulography (EMA) signals during the AAI process. We train our model using an adversarial approach and introduce an attention-based Multi-duration phoneme discriminator (MDPD) designed to fully capture the intricate relationship among multi-channel articulatory signals. Our method achieves a Pearson correlation coefficient of 0.847, marking state-of-the-art performance in speaker-independent AAI models. The implementation details and code can be found online.

==> 2_2_Related_Work.tex <==
% \section{Related work}
\section{EMA dataset}
\label{sec_ema}
Electromagnetic articulography (EMA) is a commonly used method for recording articulatory data and speech simultaneously.
Especially, in this work, we used a public dataset Haskins Production Rate Comparison (HPRC)~\cite{haskins}.
The HPRC dataset has eight native American English speakers, four females (F01-F04) and four males (M01-M04), and 720 utterances respectively.
The recorded speeches are at a rate of 44.1 kHz, and the corresponding EMA is recorded at a 100 Hz sampling rate.
The EMA data is measured using eight sensors, including tongue rear (TR), tongue blade (TB), tongue tip (TT), upper lip (UL), lower lip (LL), lower incisor (LI), mouth left (ML), and jaw left (JAWL).
Each sensor is measured in the midsagittal plane in X, Y, and Z directions, which denote movements of articulators from posterior to anterior, right to left, and inferior to superior, respectively.



